DeepSZ: Identification of Sunyaev-Zel'dovich Galaxy Clusters using Deep Learning

Galaxy clusters identified from the Sunyaev Zel'dovich (SZ) effect are a key ingredient in multi-wavelength cluster-based cosmology. We present a comparison between two methods of cluster identification: the standard Matched Filter (MF) method in SZ cluster finding and a method using Convolutional Neural Networks (CNN). We further implement and show results for a `combined' identifier. We apply the methods to simulated millimeter maps for several observing frequencies for an SPT-3G-like survey. There are some key differences between the methods. The MF method requires image pre-processing to remove point sources and a model for the noise, while the CNN method requires very little pre-processing of images. Additionally, the CNN requires tuning of hyperparameters in the model and takes as input, cutout images of the sky. Specifically, we use the CNN to classify whether or not an 8 arcmin $\times$ 8 arcmin cutout of the sky contains a cluster. We compare differences in purity and completeness. The MF signal-to-noise ratio depends on both mass and redshift. Our CNN, trained for a given mass threshold, captures a different set of clusters than the MF, some of which have SNR below the MF detection threshold. However, the CNN tends to mis-classify cutouts whose clusters are located near the edge of the cutout, which can be mitigated with staggered cutouts. We leverage the complementarity of the two methods, combining the scores from each method for identification. The purity and completeness of the MF alone are both 0.61, assuming a standard detection threshold. The purity and completeness of the CNN alone are 0.59 and 0.61. The combined classification method yields 0.60 and 0.77, a significant increase for completeness with a modest decrease in purity. We advocate for combined methods that increase the confidence of many lower signal-to-noise clusters.

==> Tables/Tables.tex <==
\begin{table}[h]
\centering
\label{tab:con_mat_all}
\begin{tabular}{lll}
\toprule
 &
\textbf{Has Cluster (Truth)} &
\textbf{No Cluster (Truth)} \\
\midrule
\textbf{Has Cluster (Predicted)} & 74.8\% & 25.2 \% \\
\textbf{No Cluster (Predicted)}  & 24.4\% & 75.6 \%  \\
\bottomrule
\end{tabular}
\medskip
\caption{Confusion matrix for the combined set, with all of the astrophysical components and instrument noise.}
\end{table}

==> Tables/tablesT.tex <==



\def \tableconfusionmatrixCNN {
% maybe we can put color in the table to help draw the eye to comparisons to make. 
\begin{table}[h]
\centering
\begin{tabular}{lll}
\toprule
 &
\textbf{Has Cluster (Truth)} &
\textbf{No Cluster (Truth)} \\
\midrule
\textbf{Has Cluster (Predicted)} & 1186 & 945 \\
\textbf{No Cluster (Predicted)}  & 659 & 102393  \\
\bottomrule
\end{tabular}
\medskip
\caption{Confusion matrix of CNN method on the test set, with threshold selected on the validation set}
\label{tab:con_mat_cnn}
\end{table}


}
